Combining Hierachical VAEs with LLMs for clinically meaningful timeline summarisation in social media

We introduce a hybrid abstractive summarisation approach combining hierarchical VAE with LLMs (LlaMA-2) to produce clinically meaningful summaries from social media user timelines, appropriate for mental health monitoring. The summaries combine two different narrative points of view: clinical insights in third person useful for a clinician are generated by feeding into an LLM specialised clinical prompts, and importantly, a temporally sensitive abstractive summary of the user's timeline in first person, generated by a novel hierarchical variational autoencoder, TH-VAE. We assess the generated summaries via automatic evaluation against expert summaries and via human evaluation with clinical experts, showing that timeline summarisation by TH-VAE results in more factual and logically coherent summaries rich in clinical utility and superior to LLM-only approaches in capturing changes over time.

==> misc/6.experiment_evaluation_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTE

% This is a backup version of the metrics;
% we keep it here since we are considering removing
% the distinction between evaluating "main" vs "changes".

% This is because there may be an inherent mismatch between
% what the LLM is prompted to generate and
% what the human annotators were instructed to summarise initially

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation}\label{evaluation} 

%We sampled thirty timelines from \citet{tsakalidis2022-identifying}'s longitudinal mental health dataset as our test set. 
We worked with three graduate students in clinical psychology, non-native fluent English speakers, to create gold-standard evidence-supported summaries from the thirty sampled timelines (\S\ref{sec:experiments.dataset}). We introduced the task over three training sessions under the supervision of a senior clinical expert. Subsequently they highlighted clinically important evidence in timelines (see Appendix, Table \ref{method.tab:clinical_concepts}) and summarised each timeline. %The same team subsequently participated in human evaluation of model-generated summaries. 

\subsubsection{Evaluation Aspects \& Metrics}\label{eval:metrics}

We peform automatic evaluations on our test set with respect to the below aspects. On metrics that require NLI, we use a \textsc{RoBERTa} model \citep{liu2020roberta} fine-tuned on fact verification, NLI, and adversarial NLI \cite{nie-etal-2020-adversarial}.\footnote{\url{https://huggingface.co/ynie/roberta-large-snli_mnli_fever_anli_R1_R2_R3-nli}} 
% MHIC

\smallskip
\noindent\textbf{Salient information preservation.} Timeline summaries should capture clinically relevant information (Table \ref{method.tab:clinical_concepts}). We adapt MHIC \cite{Srivastava20222Counseling}, but rather than computing separate scores based on hard utterance categories we compute a unified one using the semantic intersection of information highlighted by annotators (Appendix \ref{sec:appendix_intersection}), and instead of ROUGE we measure semantic similarity. Specifically, given evidence $E$ and timeline summary sentences $T$, we average the maximum recall-oriented BERTScore \cite{Zhang*2020BERTScore}:% over each $e$ in $E$:
\begin{equation*}
\text{MHIC}_{sem} = \frac{1}{|E|} \sum_{e \in E} \max_{t \in T} R_{\text{BERT}}(e, t)
\end{equation*}

% FC_Timeline
% \smallskip
\noindent\textbf{Factual consistency.} Timeline summaries should accurately reflect timeline contents, and high-level summaries should be consistent with gold-standard mental health insights. We measure whether timeline summaries are consistent with original timelines. We modify the splitting procedure used when computing faithfulness scores in traditional summarisation \citep{maynez-etal-2020-faithfulness} by splitting timeline texts with a cutoff of 60 tokens, so that texts match input lengths in the NLI model's training data. Then, given a chunked timeline $D$ and its timeline summary $T$, for every sentence $t$ in $T$, we calculate the maximum probability of a timeline chunk $d$ in $D$ entailing $t$ using a NLI model and average across all summary sentences. 
% \cite{williams-etal-2022-anlizing}

\vspace{-.5em}
\begin{equation*}
\text{FC}_\text{Timeline} = \frac{1}{|T|} \sum_{t \in T} \max_{d \in D} \text{NLI}(\text{Entail}| d, t)
\end{equation*}

Next, we measure the consistency of high-level summaries to gold high-level summaries, where consistency is the absence of contradiction. We define $C$ to be a function that quantifies the consistency of text $B$ based on text $A$.

\vspace{-1em}
\begin{equation*} 
\resizebox{1.05\hsize}{!}{$
C(A, B) = \frac{1}{|A| \cdot |B|} \sum_{a \in A} \sum_{b \in B} \left(1 - \text{NLI}(\text{Contradict}|a, b)\right)
$}
\end{equation*}

% FC_expert_m, FC_expert_c
Both gold summaries $G$ and generated summaries $S$ are split into one part that presents overall insights and one that focuses on changes in well-being. We separately score each part via $C(G', S')$. 

\smallskip
\noindent\textbf{Evidence appropriateness.} High-level mental health summaries should be consistent with their accompanying timeline summaries. We separately evaluate each high-level summary $S$'s main body $S_\text{m}$, and its section on changes $S_\text{c}$. 

First, we evaluate the main summary. We prefix every sentence $t$ in timeline summary $T$ with "The individual wrote:" to obtain $T_p$.\footnote{While we did not find statistically significant differences between the selected prefix vs. no prefix and vs. similar alternatives, we decided on prefixing as empirically it seemed to help the NLI model on noisy premises.} We measure the consistency of $S_\text{m}$ to $T_p$: $\text{EA}_\text{m} = C(T_p, S_\text{m})$. 

Next, we evaluate the summarised changes. We consider the entire timeline summary as a single multi-sentence premise and prefix it once to obtain $T'$. We compute the average probability of $T'$ entailing each sentence $s$ in $S_\text{c}$:
\begin{equation*} 
\text{EA}_\text{c} = \frac{1}{|S|} \sum_{s \in S} \text{NLI}(\text{Entail}|T', s).
\end{equation*}
\noindent\textbf{Coherence.} Summaries should present logically interconnected information sequences. %Summaries "should build from sentence to sentence to a coherent body of information" \cite{dang-2006-duc}. 
We focus on high-level summaries, as timeline summaries can naturally contain contradicting information due to user changes over time. We estimate how easy it is to follow the summary using BARTScore \cite{NEURIPS2021_e4d2b6e6}, which computes the likelihood of the summary given the source under a fine-tuned \textsc{BART} model \citep{lewis2020-bart}. We also evaluate \emph{logical} connectedness via intra-summary NLI (IntraNLI), taking the mean consistency score across each sentence against all other sentences. 
%\cite{goyal-etal-2022-snac} - error taxonomy

\smallskip
\noindent\textbf{Fluency.} %Summaries are fluent if they "have no formatting problems, capitalization errors or obviously ungrammatical sentences [...] that make the text difficult to read" \cite{dang-2006-duc}. 
We separately estimate fluency for timeline and high-level summaries using perplexity (PPL) under \textsc{GPT-2-xl} \cite{radford2019language}.

%\paragraph{Usefulness.} Summaries should help the clinician understand the client’s condition. This is assessed via human evaluation only, with respect to general usefulness and with respect to categories in Table \ref{method.tab:clinical_concepts} (diagnosis, interpersonal and intrapersonal, MoC). 

%\subsubsection{Human Evaluation}\label{eval:human}
%To elicit preferences, we select Best-Worst Scaling (BWS; \citet{louviere1991best}), an efficient ranking approach found to be reliable and suitable for detecting between-system differences \cite{kiritchenko-mohammad-2017-best}. For each test timeline, each annotator is presented with one model-generated summary per system in randomly shuffled order, and asked to select the best and worst ones based on each aspect. 

==> misc/7.results_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOTE

% This is a backup version of results;
% we keep it here since we are considering removing
% the distinction between evaluating "main" vs "changes".

% This is because there may be an inherent mismatch between
% what the LLM is prompted to generate and
% what the human annotators were instructed to summarise initially

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{ll}
\toprule
Timeline Summary & High-level Summary \\ \midrule
\begin{minipage}[t]{.9\columnwidth}%
I hate school. im so scared.i love the cat so much. i'm gonna go be counter for a while. unknown good night all! i hate my nose. fuck the sat. i got a commitment ring 3 i've got counterbodied under my eyes. i feel alone i feel like everyone hates me. i hate saying this because it sounds bad, but i really want someone to pay attention to me. solid my mom only cares about my brothers learning disabilities and her new boyfriend expressive. my boyfriend goes throug of ptsd like depression symptoms, so he gets distant sometimes levels. i literally have no friends argue. i've always been quiet but sometimes i just want someone never pay attention to me. i argue to know only when't be a body. i have to know. i'll have to be happy. %
\end{minipage}
& \begin{minipage}[t]{2\columnwidth}%
The individual is likely experiencing a range of mental health issues, including depression, anxiety, and low self-esteem. They report feeling isolated, lonely, and frustrated, with a history of stressful life events. The individual's mood appears to be low, with expressions of sadness, frustration, and anger. \\

It is evident that they have a profound craving for attention and connection with others, as well as a yearning for acceptance and validation. However, their fear of rejection and abandonment hinders them from forming and maintaining healthy relationships. Moreover, their self-criticism and preoccupation with perceived shortcomings indicate a lack of self-compassion and acceptance of their strengths and vulnerabilities.\\

The individual's mood and well-being have been observed to fluctuate over time, with both positive and negative changes experienced. The individual has expressed a range of emotions, including sadness, loneliness, and frustration, as well as moments of happiness and positivity. Noteworthy positive changes include their excitement about having a cat and receiving a commitment ring, which are associated with positive emotions and a sense of joy. However, the individual also struggles with school and experiences anxiety and depression, which are linked to negative emotions such as sadness, fear, and frustration.

\end{minipage}\tabularnewline \bottomrule
\end{tabular}
\end{adjustbox} \caption{Example TH-VAE timeline summary and its high-level summary. Examples for all systems in Appendix \ref{sec:appendix}.}
\label{tab:results.examples}
\end{table*}

\section{Results}
\label{sec:results}

\subsection{Automatic evaluation}
Table \ref{tab:results.examples} shows example summaries. For reference-based metrics, we report results averaged over the gold summaries. We perform two-tailed permutation tests in our comparisons and report statistical significance at the $\alpha=.05$ level. 

\begin{table}[!htbp]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}llrrr@{}}
\toprule
Aspect & Metric & LLaMA & TH-VAE & Skeleton \\ \midrule
% salient meaning preservation
SMP 
    & $\text{MHIC}_\text{sem}$ & .656 & \textbf{.661} & .572 \\
    % for "comparison" vs Srivastava et al 2022, the ROUGE-1 MHIC results are: .387, .452, .395
% factual consistency
\multirow[t]{3}{*}{FC} 
    & $\text{FC}_\text{Timeline}$ & \textbf{.634} & .632 & .216 \\
    % we originally binarised the probabilities,
    % but since the domain + data splitting are different from Maynez 2020 already, here we report the non-binarised probabilities
    % binarised results are: .4, .7, 0
    & $\text{FC}_\text{Expert-m}$ & \textbf{.964} & .963 & .959 \\
    & $\text{FC}_\text{Expert-c}$ & .933 & .937 & \textbf{.941} \\
 % evidence appropriateness
\multirow[t]{2}{*}{EA} 
    & $\text{EA}_\text{m}$ & \textbf{.972} & .971 & .955 \\
     & $\text{EA}_\text{c}$ & .424 & .414 & \textbf{.503}\\ 
 % coherence
\multirow[t]{2}{*}{Coherence} 
    & IntraNLI & .956 & \textbf{.963} & .957 \\
    & BARTScore & \textbf{-2.96} & -3.10 & -3.09 \\
 % fluency
\multirow[t]{2}{*}{Fluency} 
 & $\text{PPL}_\text{Timeline}$ ($\downarrow$) & \textbf{\underline{13.80}} & 56.33 & 31.82 \\
 & $\text{PPL}_\text{High-level}$  ($\downarrow$)& 9.32 & \textbf{9.30} & 9.45 \\ \hline 
\end{tabular} 
\end{adjustbox}
\caption{Automatic evaluation results for salient meaning preservation (SMP), factual consistency (FC), evidence appropriateness (EA), coherence, and fluency. Higher is better, except for PPL. Best in \textbf{bold}, significant improvement over second-best in \underline{underline}.} 
\label{tab:results.auto}
\end{table}


\smallskip
\noindent\textbf{TH-VAE generates factually consistent and coherent summaries that capture mental health phenomena over time.} We found TH-VAE summaries to be the most factually consistent to the original timelines, as shown in Table \ref{tab:results.auto}. High-level summaries generated from TH-VAE evidence were the most consistent with gold mental health insights ($\text{FC}_\text{Expert-m}$), most logically coherent (IntraNLI), and ties with LLaMA as the best model in terms of preserving mental health information ($\text{MHIC}_{sem}$). 

\smallskip
\noindent\textbf{LLaMA-based summaries are fluent but less consistent with timeline data.} 
LLaMA produced summaries are the most fluent (Table \ref{tab:results.auto}). The discrepancy between $\text{MHIC}_{sem}$ and $\text{FC}_\text{Timeline}$ scores suggest that LLaMA timeline summaries excel in recall of mental health information but may fall short in precision. $\text{FC}_\text{Expert-c}$ scores indicate consistency with expert observations on changes, however permutation tests did not reveal a statistically significant difference among the three systems.

\noindent\textbf{Prompting enables generation of fluent mental health insights grounded in summarised timeline evidence.} Overall, mental health insights in high-level summaries across systems are generally consistent with their respective timeline summaries, based on $\text{EA}_\text{m}$ and $\text{EA}_\text{c}$ (Table \ref{tab:results.auto}). High-level summaries are comparably fluent with no significant difference in PPL, which is as expected given that they were produced using the same prompting model and framework. 

Permutation tests did not reveal statistically significant differences between systems in terms of consistency with gold summaries of changes ($\text{FC}_\text{Expert-c}$), despite more pronounced gaps in other metrics related to capturing mental health insights. Given that all systems used key phrases that were few-shot prompted with expert examples, an explanation is that such phrases served as anchors for capturing changes across modelling strategies. We plan to explore how to effectively incorporate expert insights in prompting for temporally-sensitive tasks in future work.

\subsection{Ablation}
We performed ablation studies to investigate the importance of the key phrases (\S\ref{method:key}) and the elaborate clinical prompts for the final summary generation (\S\ref{method:summary}). 
We hypothesize that the key phrases can guide the TH-VAE to generate the mental health related timeline summary. Therefore, when generating the timeline summary, we use key phrases to highlight key information in the timeline. To test the contribution of key phrases, we remove the key phrases when generating timeline summary for comparison. Furthermore, we also tested whether our proposed clinical prompts can guide the LLM to generate the high-level summary with clinical insights (e.g., diagnosis, inter- and intra- personal aspects, moments of change). 
In particular, we experimented with (a) removing key phrases but keeping the clinical prompts ('TH-VAE \textit{-keyphrases}') and (b) keeping the key phrases, but prompting the LLM to summarise the high-level summary directly without any guiding questions/topics ('TH-VAE \textit{-clinical prompts}').


\begin{table}[!htbp]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}llrrr@{}}
\toprule
Aspect & Metric & TH-VAE & \makecell[c]{TH-VAE \\ \textit{-keyphrases}} & \makecell[c]{TH-VAE \\ \textit{-clinical prompts}} \\ \midrule
% salient meaning preservation
SMP 
    & $\text{MHIC}_\text{sem}$ & \textbf{.661} & .621 & \textbf{.661} \\
    % for "comparison" vs Srivastava et al 2022, the ROUGE-1 MHIC results are: .387, .452, .395
% factual consistency
\multirow[t]{3}{*}{FC} 
    & $\text{FC}_\text{Timeline}$ & \textbf{.632} & 525 & \textbf{.632} \\
    % we originally binarised the probabilities,
    % but since the domain + data splitting are different from Maynez 2020 already, here we report the non-binarised probabilities
    % binarised results are: .4, .7, 0
    & $\text{FC}_\text{Expert-m}$ & \textbf{.963} & .954 & .923 \\
     & $\text{FC}_\text{Expert-c}$ & .937 & \textbf{.954} & .931 \\
 % evidence appropriateness
\multirow[t]{2}{*}{EA} 
    & $\text{EA}_\text{m}$ & \textbf{.971} & .938 & .938 \\
    & $\text{EA}_\text{c}$ & .414 & .475 & .292 \\ 
 % coherence
\multirow[t]{2}{*}{Coherence} 
    & IntraNLI & \textbf{.963 }& .952 & .939 \\
    & BARTScore & -3.105 & -3.083 & \textbf{-2.744} \\
 % fluency
\multirow[t]{2}{*}{Fluency} 
 & $\text{PPL}_\text{Timeline}$ ($\downarrow$) & \textbf{56.337} & 81.451 & \textbf{56.337} \\
 & $\text{PPL}_\text{High-level}$  ($\downarrow$)& \textbf{9.304} & 9.385 & 13.629 \\ \hline 
\end{tabular} 
\end{adjustbox}
\caption{Ablation study: Automatic evaluation results. Best in \textbf{bold}} 
\label{tab:ablation}
\end{table}

Tables~\ref{tab:ablation} shows the experiment results. When keyphrases are removed, timeline summaries preserve less salient information ($\text{SMP}$) and are less consistent ($\text{FC}_\text{timeline}$) with the source timeline. The removal of keyphrases also degraded the logical connectedness ($\text{IntraNLI}$), evidence appropriateness ($\text{EA}$), and factual consistency with gold summaries ($\text{FC}_\text{expert}$). This shows that the keyphrases help TH-VAE to capture mental health related information from the timeline. Furthermore, we observed the same trend to a greater extent when we removed clinical prompts. Resulting summaries were less logically connected ($\text{IntraNLI}$), achieved lower evidence appropriateness ($\text{EA}$) and were less consistent with gold summaries ($\text{FC}_\text{expert}$). Therefore, the elaborate prompt dose provide an efficient guidance for the LLM to generate summary in terms of clinical aspects.




% This section is in progress and will be updated by morning of Thursday 14 Dec
\subsection{Human evaluation}
We select the top three performing models for human evaluation. 

(Table goes here)

Table (PLACEHOLDER) reports the human evaluation results.

Consistent with automatic evaluation, TH-VAE produced summaries that were considered the most factually consistent and useful in summarising changes among the compared models. 
LLaMA summaries generated with clinical prompts were considered more useful in other usefulness criteria, whereas LLaMA with a simple summarisation prompt were rated the lowest across the board in terms of usefulness.
Notably, human judges found LLaMA summaries generated \emph{without} clinical prompts to be more factually consistent than those \emph{with} clinical prompts, suggesting they synthesised the source timeline's content faithfully but fell short in clinical usefulness due to lack of guidance.





%% Previous BWS results - data as of 14 Oct 2023 (old data)
%\begin{table}[!htbp]
%\begin{adjustbox}{width=\columnwidth}
%\begin{tabular}{@{}lccc@{}}
%\toprule 
%Aspect                                      & LLaMA & TH-VAE & Skeleton \\ \midrule
%Salient Meaning Preservation                & \textbf{.80} & .44  & .26 \\
%Factual Consistency                         & \textbf{.63} & .54  & .32    \\
%Evidence Appropriateness                    & \textbf{.74} & .45  & .29    \\
%Coherence                                   & .43 & .43 &  \textbf{.62} \\
%Fluency                                     & \textbf{.60}   &  .46 &  .44     \\
%Usefulness (Overall)                        & \textbf{.77}   &  .50 & .22  \\ 
%\phantom{----}(Diagnosis)                      & \textbf{.77}  &  .50 & .22  \\
%\phantom{----}(Inter-\& Intrapersonal) & \textbf{.64}  &  .47 & .37    \\
%\phantom{----}(MoC)                            & .50   &  \textbf{.66} & .33  \\ \bottomrule
%\end{tabular}
%\end{adjustbox}
%\caption{Human evaluation results based on Best-Worst Scaling. Best in \textbf{bold}. (TODO - \textcolor{red}{Results all subject to change; based on 30 timelines from annotator A, 10 timelines each from B, C (missing 40/90 data points)})}
%\label{tab:results.bws}
% note - first 2 decimals are indeed the same for overall and diagnosis; have checked
%\end{table}

==> misc/7.results_outdated.tex <==
\section{Results}
\label{sec:results}

\subsection{Automatic evaluation}
Table \ref{tab:results.examples} shows example summaries. %For reference-based metrics, we report results averaged over the gold summaries. 
We perform two-tailed permutation tests in our comparisons reporting statistical significance at $\alpha=.05$. 

\begin{table}[]

\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}llrrrr@{}}
\toprule
Aspect & Metric & LLaMA & TH-VAE & Skeleton \\ \midrule
% salient meaning preservation
SMP 
    & $\text{MHIC}_\text{sem}$ & .65 & \textbf{.66} & .57 \\
% factual consistency
\multirow[t]{3}{*}{FC} 
    & $\text{FC}_\text{Timeline}$ & \textbf{.63} & \textbf{.63} & .21 \\
    & $\text{FC}_\text{Expert}$ & .95 & \textbf{.96} & .95 \\
 % evidence appropriateness
\multirow[t]{2}{*}{EA} 
    & $\text{EA}$ & \textbf{.97} & \textbf{.97} & .95 \\
 % coherence
\multirow[t]{2}{*}{Coherence} 
    & IntraNLI & .95 & \underline{\textbf{.96}} & .95 \\
    & BARTScore & \textbf{-2.96} & -3.10 & -3.09 \\
 % fluency
\multirow[t]{2}{*}{Fluency} 
 & $\text{PPL}_\text{Timeline}$ ($\downarrow$) & \underline{\textbf{13.80}} & 56.33 & 31.82 \\
 & $\text{PPL}_\text{High-level}$  ($\downarrow$)& 9.32 & \textbf{9.30} & 9.45 \\ \hline 
\end{tabular} 
\end{adjustbox}
\caption{Automatic evaluation results for salient meaning preservation (SMP), factual consistency (FC), evidence appropriateness (EA), coherence, and fluency. Higher is better, except for PPL. Best in \textbf{bold}, significant improvement over second-best in \underline{underline}. %Naive prompting baseline directly produces high-level summaries without an intermediate timeline summary, hence the lack of results on timeline-level metrics.
} 
\label{tab:results.auto}
\vspace{-1.5em}
\end{table}


TH-VAE and LLaMA generated significantly higher quality summaries compared to skeleton. %other baselines. 
TH-VAE and LLaMA were comparable on most metrics, preserving mental health information ($\text{MHIC}_{sem}$) while achieving similar consistency with the source  ($\text{FC}_\text{Timeline}$) in timeline summaries, and achieving similar factual consistencies to human-written references in high-level mental health summaries ($\text{FC}_\text{Expert}$). However, while permutation tests revealed LLaMA timeline summaries to be significantly more fluent ($\text{PPL}_\text{Timeline}$), TH-VAE summaries were significantly more internally logically coherent (IntraNLI). 

%Systems which leverage keyphrases and clinical prompts %(LLaMA, TH-VAE, Skeleton) 
Systems were relatively comparable on consistency with expert summaries ($\text{FC}_\text{Expert}$) despite more pronounced gaps in other metrics ($\text{FC}_\text{Timeline}$, MHIC). This suggests the combination of keyphrases prompted with expert examples and prompts informed by clinical expertise served as anchors for capturing and synthesising mental health signals across modelling strategies. %We plan to explore how to effectively incorporate expert insights in prompting for temporally-sensitive tasks in future work.

\subsection{Human evaluation}

We selected the two best systems, LLaMA and TH-VAE, for human evaluation with expert annotators. Annotators scored the summaries on a 5-point Likert scales (1 is worst, 5 is best) based on criteria outlined in Appendix D. Qualitative discussion of the summaries by a senior clinical expert can be found in Appendix \ref{sec.appendix.qualitative}. As shown in Table \ref{tab:results.likert}, TH-VAE produced summaries considered more factually consistent and useful in summarising changes (MoC). Human judges found LLaMA summaries to be more useful in other usefulness criteria. 

\begin{table}[!htbp]
\centering
\begin{adjustbox}{width=.75\columnwidth}
\begin{tabular}{@{}lccc@{}}
\toprule 
Aspect                                      & LLaMA & TH-VAE \\ \midrule
Factual Consistency                         & 3.08 & \textbf{3.35}   \\
Usefulness (General)      & \textbf{3.38} & 3.28  \\
\phantom{---} (Diagnosis) & \textbf{3.40} & 3.25   \\
\phantom{----}(Inter-\& Intrapersonal) & \textbf{3.48}  &  3.33    \\
\phantom{----}(MoC)       & 3.30   &  \textbf{3.35}  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Human evaluation results %based on 5-point Likert scales (5 is Best). 
Best in \textbf{bold}.}
\label{tab:results.likert}
\vspace{-1em}
\end{table}

\vspace{-0.1cm}
\subsection{Ablation} \label{ap:ablation}
We performed ablation studies to investigate the importance of key phrases (\S\ref{method:key}) and elaborate clinical prompts for the final summary generation (\S\ref{method:summary}) in TH-VAE.  %indicates the necessity of first generating a timeline summary and then generating a high-level summary, instead of directly using the timeline to generate the summary.
% In addition, we also explored the importance of keyphrases, timeline summary and clinical prompt in Naive Llama. 
%For TH-VAE,w
We experimented with (a) removing keyphrases but keeping the clinical prompts (`\textit{-keyphrases}') and (b) keeping the keyphrases, but prompting the LLM to summarise the high-level summary directly without any guiding topics (`\textit{-clinical prompts}'). 
% For Naive Llama, we (a) generate timeline summary without keyphrases, but keep clinical prompt (`\textit{-keyphrases}'), (b) generate high-level summary with timeline directly (`\textit{-timeline sum}'), (c) keep timeline summary, but remove clinical prompt (`\textit{-clinical prompts}').
When keyphrases are removed, timeline summaries preserve less salient information ($\text{SMP}$) and are less consistent ($\text{FC}_\text{Timeline}$) with the source timeline. It also degraded the logical connectedness ($\text{IntraNLI}$), evidence appropriateness ($\text{EA}$), and factual consistency ($\text{FC}_\text{Expert}$), showing that keyphrases help TH-VAE capture mental health related information. We observed the same trend to a greater extent when clinical prompts are removed. Thus, the elaborate prompt dose provide an efficient clinical guidance for the LLM to generate summaries. %Details are in Appendix, Table~\ref{tab:ablation}. 
% \ref{ap:ablation}. 
% Additionally results for Naive in Tables~\ref{tab:results.auto},~\ref{tab:results.likert} show the importance of timeline summarisation, lacking in Naive Llama.




==> the_version_of_changes/1.abstract.tex <==
\begin{abstract}

\textcolor{blue}{We introduce a hybrid abstractive summarisation approach combining hierarchical VAE with LLMs (LlaMA-2) to produce clinically meaningful summaries from social media user timelines, appropriate for mental health monitoring. 
The summaries combine two different narrative points of view: clinical insights in third person useful for a clinician are generated by feeding into an LLM specialised clinical prompts, and importantly, a temporally sensitive abstractive summary of the user's timeline in first person, generated by a novel hierarchical variational autoencoder, TH-VAE.
We assess the generated summaries via automatic evaluation against expert written summaries and via human evaluation with clinical experts, showing that timeline summarisation by TH-VAE results in more factual and logically coherent summaries rich in clinical utility and superior to LLM-only approaches in capturing changes over time.}
\iffalse
We introduce the new task of clinically meaningful summarisation of social media user timelines, appropriate for mental health monitoring. We develop a novel approach for unsupervised abstractive summarisation that produces a two-layer summary consisting of both \textit{high-level} information, covering aspects useful to clinical experts, as well as accompanying time sensitive \textit{evidence} from a user's social media timeline. 
A key methodological novelty comes from the
timeline summarisation component based on a version of hierarchical variational autoencoder (VAE) adapted to represent long texts and guided by LLM-annotated key phrases. 
The resulting timeline summary is input into a LLM (LLaMA-2) to produce the final summary containing both the high level information, obtained through instruction prompting, as well as corresponding evidence from the user's timeline. 
We assess the summaries generated by our novel architecture via automatic evaluation against expert written summaries and via human evaluation with clinical experts, showing that timeline summarisation by TH-VAE results in logically coherent summaries rich in clinical utility and superior to LLM-only approaches in capturing changes over time.


We develop a novel approach for unsupervised abstractive summarisation that produces a two-layer summary consisting of both \textit{high-level} information, covering aspects useful to clinical experts, as well as accompanying time sensitive \textit{evidence} from a user's social media timeline. 
A key methodological novelty comes from the
timeline summarisation component based on a version of hierarchical variational autoencoder (VAE) adapted to represent long texts and guided by LLM-annotated key phrases. 
The resulting timeline summary is input into a LLM (LLaMA-2) to produce the final summary containing both the high level information, obtained through instruction prompting, as well as corresponding evidence from the user's timeline. 
\fi

\end{abstract}



==> the_version_of_changes/10.Limitation.tex <==
\section*{Limitations}
Our work considers the segmentation of timelines in terms of
moments of change as changes in an individual’s
mood judged on the basis of their self-disclosure
of their well-being. This is faced by two limiting
factors: (a) users may not be self-disclosing important aspects of their daily lives and (b) while also \cite{hills-etal-2023-creation} segment user timelines based on moments of change in mood there may be other appropriate ways to effectively segment timelines into semantically related temporal units. For example timelines could be segmented based on symptoms or life events which could also be evolving over time. Empirically we have not found topics to be an effective way of identifying sub-timelines and segments within a timeline but the best way of segmenting the timelines is an open research direction. 

Though our models could be tested in cases of nonself-disclosure (given the appropriate ground truth labels), the analysis and results presented in this
work should not be used to infer any conclusion on such cases. 

While we believe our methods for clinically meaningful longitudinal summarisation of social media data for mental health monitoring to be applicable to non-social media longitudinal data such as therapy sessions, this remains future work. 


\textcolor{blue}{In the present study, we have conducted a comparison between timeline summarization using TH-VAE, skeleton-based and LLM-generated summaries. A further qualitative evaluation by a senior clinical therapist found that the summaries generated by Llama often reached conclusions that were not sufficiently supported by the evidence provided in the timeline, and were lower in factual consistency than the TH-VAE. The TH-VAE and Llama were effective in summarizing the intrapersonal and interpersonal patterns and moments of change, but their depiction of diagnostic aspects was only moderately accurate, characterized by some inaccuracies and omissions. These findings will help pinpoint areas where our models can be enhanced and refined. }


==> the_version_of_changes/2.introduction.tex <==
\subsection{Introduction}


Social media users discuss different aspects of their lives, providing important clues about their mental health.
Previous work \cite{de2013predicting, coppersmith2014quantifying, cohan2018-smhd, chancellor2020methods} have studied users' social media posts to help identify depression, bipolar disorder \cite{yates2017-depression,husseini2018-deep} or self-harm \cite{zirikly2019clpsych}, and there have been efforts on multi-task learning to capture user states at a particular moment in time \cite{benton-etal-2017-multitask, yang-etal-2023-towards}. Despite the importance of longitudinal assessments of linguistic and other digital content for mental health clinical outcomes \cite{velupillai2018using}, there is little work on considering the evolution of an individual's mental health over time through their social media. 
\citet{tsakalidis2022-identifying, tsakalidis2022-overview} established the task of capturing changes (switches and escalations) in an individual's mood over time and showed how identifying these helps predict clinical assessments of suicidal ideation. 
However, currently clinicians don't have access to such information to assess individuals' mental-state and they mainly rely on self-reports completed by patients throughout psychotherapy \cite{crits2021psychotherapy}. 
Although standardized subjective measures are fundamental to mental health monitoring and research, they have significant limitations, such as the extent of individuals’ self-awareness, their willingness to complete questionnaires, and the limited choice of responses \cite{kazdin2021extending}. 
\textcolor{blue}{Providing concise summaries that can capture fluctuations in individuals' state-of-mind while emphasizing key clinical concepts, can significantly assist in monitoring, prevention and early detection of mental health issues. Such summaries would augment clinician capacity, provide alternatives to standard questionnaires and compensate for reduced access to mental health services \cite{schwartz2023assessments}. }


\textcolor{blue}{To the best of our knowledge we are the first to propose clinically meaningful summaries of social media user `timelines' (sequences of chronologically ordered posts by a user). Driven by the need to concisely summarise time-series language data which can span arbitrary lengths that exceed limits of many contemporary models and render purely extractive methods impractical, we propose a novel hybrid unsupervised abstractive method, Timeline Hierarchical VAE (TH-VAE). Our system makes use of a hierarchical variational autoencoder that compresses timeline information into compact representations and a large language model (LLM), creating a two-layer summary that combines two different narrative points of view. Specifically: a \textit{high-level} summary in third person useful for a clinician, is generated by feeding into an LLM specialised clinical prompts and importantly a temporally sensitive abstractive summary of the user's timeline in first person (\textit{evidence summary}), generated by TH-VAE. %accompanied by temporally sensitive \textit{evidence} from the user's timeline. 
The generation of the first person abstractive evidence summary via TH-VAE is guided by mental health related key-phrases obtained through instruction prompting by an LLM.
The final resulting high level summary covers aspects considered to be crucial by clinicians from a wide range of therapeutic approaches, including individuals' diagnosis, intrapersonal and interpersonal patterns and extent of mental state changes over time \cite{eells2022handbook}.\footnote{For a complete list, please see Table \ref{tab:appendix.clinical_concepts} in Appendix \ref{sec:appendix}.} }

\noindent We make the following contributions:

\squishlist
\item \textcolor{blue}{We develop a novel abstractive timeline summarisation method (TH-VAE) based on adapting a hierarchical VAE model (NVAE)(\S\ref{method:h_vae}) to longitudinal social media data (user timelines). }

\item \textcolor{blue}{We provide a new task, the creation of clinically meaningful summaries from social media data. These summaries, generated in a hybrid approach, comprise high-level information in third person consistent with clinical insights (diagnosis, inter- and intra- personal aspects, moments of change) and evidence from a user's timeline, generated from the TH-VAE, supporting the assigned high-level insights. (\S\ref{method})}

\item We create a dataset of expert-written mental health summaries from longitudinal social media data. A small sample of these is used to help with modeling (\S\ref{method:summary}) and the rest is used for evaluation (\S\ref{evaluation}).

\item We provide a novel detailed evaluation method of the summaries based on preservation of clinical information, summary consistency, and usefulness to clinicians, using semantic similarity based metrics, NLI based inference, as well as expert human evaluation 
(\S\ref{evaluation}).

\item We conduct experiments using different unsupervised summarisation methods based on LLMs and story generation (\S\ref{exp:baseline}), showing superior performance for our proposed TH-VAE method (\S\ref{sec:results}).


\squishend








==> the_version_of_changes/4.methodology.tex <==
\section{Methodology}\label{app.method}

\textbf{Task}\label{task}
 Given a user's timeline (a series of posts between two dates \cite{tsakalidis2022-identifying}), the goal is to generate an abstractive summary that reflects the user's mental state and how it changes over time. \textcolor{blue}{This summary includes high-level information useful for clinicians in third person, and corresponding evidence from the timeline in first person.}


\begin{figure}
\centering
\includegraphics[width=\columnwidth]{images/high-level_prompt.pdf}
\caption{Prompting framework for generating high-level summaries. Taking a first-person summarised timeline as input, we (1) prompt the LLM around different clinical topics, (2) summarise extracted inferences into prose per topic, and (3) combine the topic-specific intermediate summaries into a coherent, distilled document.} 
\label{app.fig:high_level_prompt}
\vspace{-1em}
\end{figure}


\subsection{Architecture Overview}\label{app.architecture_overview}
Fig.~\ref{app.fig:high_level_prompt} shows the summary generation process. It consists of two sub-processes:\\
(1) Abstractive generation of the timeline/evidence summary (\S\ref{app.method:h_vae}). We use three different unsupervised methods for creating the timeline summary in first person: Timeline hierarchical VAE (TH-VAE \S\ref{app.task:segments}), our key methodological novelty; LLaMA (\S\ref{exp:baseline}); a method from story generation (\S\ref{exp:baseline}).\\
(2) Generation of the High-level summary (\S\ref{method:summary}). We feed the generated timeline/evidence summary into an instruction-tuned LLM (Llama), where prompts originate from a small sample of expert human annotation (\S\ref{task:segments}), and generate high-level summaries covering clinical aspects such as diagnosis, inter- and intra- personal relationships and fluctuations in mood. 

The following subsections describe our novel timeline summarisation method using an adapted hierarchical VAE (TH-VAE).

\begin{figure}
\centering
\includegraphics[width=.8\linewidth]{images/timeline.png}
\caption{Each timeline is separated into several segments based on 'MoC'. We \hl{highlight} the key phrases.}
\label{app.timeline}
\vspace{-0.5cm}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=.88\textwidth]{images/h-vae.png}
\caption{Overview of TH-VAE. The left of the dotted line shows the construction of the k-sentence representation used only during generation, informed by the key-phrases, while the right side shows the hierarchical structure of TH-VAE, and its components.\textcolor{blue}{\ding{172} and \ding{173} represent the input during training and generation respectively.}}
\vspace{-1em}
\label{app.fig:h-vae}
\end{figure*}

\subsection{Input to Timeline Summarisation}\label{app.task:segments}
The input to TH-VAE and the other timeline summarisation methods is a user's timeline, annotated with Moments of Change in mood (MoC)\cite{tsakalidis2022-identifying}. MoC annotations consist of \textit{Switches} (sudden mood shifts, denoted by `IS'--In Switch-- and `ISB'--In Switch Beginning-- tags),  and \textit{Escalations} (gradual mood progression, denoted by `IE'--In Escalation-- and `IEP'--In Escalation Peak-- tags).
We split the whole timeline (see Fig.~\ref{app.timeline}) into several segments (sub-timelines) based on 'MoC', 
so that consecutive posts with the same label (`IE' or `IEP'),(`ISB' or `IS') or `0' are grouped together. This assumes each segment consists of posts of a similar mood type, which facilitates capturing different features and relations between them. This is somewhat similar to news timeline summarisation which clusters around stories or events, with the additional challenge that mood features are more evasive and we hope to model these through latent variables.\\
\textbf{Key phrases}\label{app.method:key} We asked clinical psychologists to annotate key phrases indicative of users' mental health in three timelines. These phrases include mood related clues but also information on interpersonal relationships, behaviors or events related to a user's mental state (see highlights in Fig.~\ref{app.timeline}). We take these annotated timeline/key phrases pairs as examples and prompt LLaMA \cite{touvron2023llama} to annotate the rest of the timelines. 
\textbf{Timeline summary representation}\label{app.method:summary_rep} For each segment ${s}_{i}$, we input its corresponding key phrase sequence $\left\{\boldsymbol{e}_{1}, ... , \boldsymbol{e}_{j}, ... , \boldsymbol{e}_{n}\right\}$ into a GRU encoder~\cite{cho2014learning} to get the key phrases encoding ${\boldsymbol{v}}=GRU(\left[\boldsymbol{e}_{1}; ... ;\boldsymbol{e}_{n}\right])$, which is represented by the last hidden state of the GRU (see left part of Fig\ref{app.fig:h-vae}). 
We calculate the similarity between ${\boldsymbol{v}}$ and each word embedding $\boldsymbol{w}_{i}$ in the segment as the weight $\alpha_{i}$: %The weight $\alpha$ of each word is defined as:
\begin{equation*}
    \begin{aligned}
    {\alpha_{i}} = \frac{cos(\boldsymbol{v}, \boldsymbol{w}_{i})}{\sum_{i^{\prime}=1}^{m}cos(\boldsymbol{v}, \boldsymbol{w}_{i^{\prime}})}.
    \end{aligned} 
\end{equation*}

Thus ${s}_{i}$ can be represented by a series of weighted word embeddings $\left\{\alpha_{1}\boldsymbol{w}_{1}, \alpha_{2}\boldsymbol{w}_{2}, ... , \alpha_{m}\boldsymbol{w}_{m} \right\}$, where ${m}$ is the length of ${s}_{i}$. We encode it with the GRU encoder to get the segment representation ${\boldsymbol{s}_{enc_{i}}}$=$GRU(\left[\alpha_{1}\boldsymbol{w}_{1}; \alpha_{2}\boldsymbol{w}_{2}; ... ; \alpha_{m}\boldsymbol{w}_{m} \right])$. 
If the timeline is divided into $k$ segments, we can get $k$ segment encodings ${s}_{enc_1},...,{s}_{enc_k}$ in this way. We concatenate these encodings in chronological order to get a segment sequence $\left\{\boldsymbol{s}_{{enc}_{1}}, \boldsymbol{s}_{{enc}_{2}}, ... , \boldsymbol{s}_{{enc}_{k}}\right\}$, apply an average pooling operation (Avg Pool)\cite{Lin2013NetworkIN} over the output of the GRU encoder~(See right part of Fig\ref{app.fig:h-vae}) and feed it into the hierarchical part of TH-VAE to generate a timeline summary.  

\subsection{Overview of TH-VAE}
Due to the lack of gold summaries for training purposes, we have to construct the summary distribution without any guidance. 
Thus we need a model that can learn an expressive distribution for a long timeline (the longest timeline has 124 posts, and the longest of these posts has over 300 words). We also need to construct a mental health related summary distribution that can capture different features and establish the long-range dependencies between these features in the timeline.
We propose TH-VAE, an unsupervised abstractive timeline summarization model adapted from NVAE \cite{vahdat2020nvae}, to construct a more expressive prior for a user timeline. 

\vspace{-0.05cm}
In the learning process, we split the timeline into several segments (sub-timelines, \S\ref{app.method:h_vae}), considered to contain consecutive posts with similar mood, and train TH-VAE to learn the distribution of each segment ${s}$ by reconstructing it.
%make TH-VAE learn the distribution for these segments. 
The latent variable of each segment is partitioned into several sub-latent variables through the hierarchical structure of TH-VAE. These sub-latent variables can capture different sub-features and establish long-range dependencies between segments in the timeline. Therefore, the final latent variable for each segment is denoted as: $\boldsymbol{z}=\left\{\boldsymbol{z}_{1}, \boldsymbol{z}_{2}, ... , \boldsymbol{z}_{l} \right\}$. 

\vspace{-0.05cm}
 When generating the evidence summary, we still treat each segment as a unit. To help the model focus on important information during generation we introduce the notion of key phrases (\S\ref{app.method:key}). We use an automatic method based on an LLM to extract mental health related key phrases from each segment and encode key phrase-segment pairs with an attention mechanism. We concatenate the sequence of segment representations of a timeline in chronological order and input it into the hierarchical structure of TH-VAE to generate the timeline/evidence summary (See~ Fig.~\ref{app.fig:h-vae}, left part).

\vspace{-0.3cm}
\subsection{Document Reconstruction via TH-VAE}\label{app.method:h_vae}

% A Variational Auto-Encoder 
\textcolor{blue}{The vanilla VAE assumes a prior $p(\boldsymbol{z})$ of document $\boldsymbol{x}$ over latent variables $\boldsymbol{z}$ to be a Normal Gaussian distribution, and parameterizes an approximate posterior distribution ${q_{\phi}(\boldsymbol{z}|\boldsymbol{x})}$ given text $\boldsymbol{x}$. It uses KL (Kullback–Leibler divergence) to calculate the distance between $p(\boldsymbol{z})$ and ${q_{\phi}(\boldsymbol{z}|\boldsymbol{x})}$ and gradually reduces the distance between them in training. Finally, it samples from the hypothesised posterior distribution and generates the document $\boldsymbol{x}$. It has been shown that the vanilla VAE can lead to over-regularising the posterior distribution, resulting in latent representations that do not represent well the structure of the data \cite{klushyn2019learning, alemi2018fixing, sonderby2016ladder, ranganath2016hierarchical, vahdat2020nvae}.
However, for a long document assuming its distribution to be a Gaussian does not provide enough expressive power; we need to be able to consider the structure of different semantic elements and the relationship between them.}

\textcolor{blue}{The deep Hierarchical VAE (NVAE) \cite{vahdat2020nvae}, introduced for images, increases expressiveness by introducing several latent variables to generate large high-quality images, demonstrates the superiority of the hierarchical VAE.
Here, we adapt this model for long documents, resulting in Timeline Hierarchical VAE (TH-VAE), and use it as the basis of constructing mental health related timeline representations. }

\subsubsection{Hierarchical Component}\label{app.sec:hierarchical}
TH-VAE increases the expressiveness of the approximate posterior and prior by partitioning the latent variable $\boldsymbol{z}$ into $l$ latent variables  $\boldsymbol{z}$=$\left\{\boldsymbol{z}_{1}, \boldsymbol{z}_{2}, ... , \boldsymbol{z}_{l} \right\}$\cite{vahdat2020nvae}. The prior is represented by ${{p(\boldsymbol{z})}={\prod_{l}{p(\boldsymbol{z}_{l}|\boldsymbol{z}_{<l})}}}$ and it parameterises the approximate posterior distribution ${q_{\phi}(\boldsymbol{z}|\boldsymbol{x})}={\prod_{l}{q_{\phi}(\boldsymbol{z}_{l}|\boldsymbol{z}_{<l},\boldsymbol{x})}}$ which are represented by factorial Normal distributions. This objective is to maximise its lower bound as:
\begin{equation*}
    \begin{aligned}
    {L(\theta;\boldsymbol{x})} = {-KL({q_{\phi}(\boldsymbol{z}_{1}|\boldsymbol{x})||p(\boldsymbol{z}_{1})})}\\
    \sum_{l=2}^{L}{\mathbb{E}_{q_{\phi}(\boldsymbol{z}<l|\boldsymbol{x})}\lbrack {-KL({q_{\phi}(\boldsymbol{z}_{l}|\boldsymbol{x},\boldsymbol{z}<l) || p(\boldsymbol{z}_{l}|\boldsymbol{z}<l)})} \rbrack}\\
    +{\mathbb{E}_{q_{\phi}(\boldsymbol{z}|\boldsymbol{x})}\lbrack {\log{p_{\theta}(\boldsymbol{x}|\boldsymbol{z})}} \rbrack}.\\ \label{app.vae_loss}
    \end{aligned}
    \vspace{-0.5cm}
\end{equation*}
\noindent \textcolor{blue}{Before going into the hierarchical architecture, we use a GRU encoder to encode the segment, to reduce the impact from padding. Then we add an Avg Pool \cite{Lin2013NetworkIN} over the output of the GRU encoder to fix the input length. Both TH-VAE and NVAE use multiple residual cells to construct the hierarchical structure. In TH-VAE we simplify residual cells to work with textual data rather than images, and keep the optimization strategies in NVAE, i.e., BN (batch normalization) with Swish Activation and Squeeze and Excitation (SE). We use two different residual cells: $residual\,cell_{1}$ and $residual\,cell_{2}$.  
The input representations first go through a \textbf{block} which focuses on capturing the features of a segment and consists of $residual\,cell_{1}$. 
To form $residual\,cell_{1}$ we use series BN, $conv$ (CNN with one kernel size), SE as well as $conv_{mul}$ (CNN with multiple kernel sizes), where the latter helps with capturing the different features. 
Then, the output of the \textbf{block} will go into the layered \textbf{group}s (see Fig.~\ref{app.fig:h-vae}--right), responsible for learning to capture the relationship between different features in segments and long-range dependencies between them. 
Each \textbf{group} is used to encode the sub-latent variables $\textbf{z}_{i}$ and consists of $residual\,cell_{2}$s. Since $conv_{mul}$ increased parameters without added benefit, we only use $conv$ in $residual\,cell_{2}$. Finally we add another \textbf{block} to integrate information.
During training, the whole hierarchical architecture is used to learn the distribution of each segment, by learning features and long-range dependencies within them via segment reconstruction (as shown in the right part of Fig\ref{app.fig:h-vae}). Then during generation a sequence of segments (a whole timeline) is input to TH-VAE to generate similarly structured text. The left part of Fig\ref{app.fig:h-vae} shows the process of encoding the sequence of segments. When decoding, we use the same decoder component as in \cite{song2022unsupervised}, consisting of a transformer decoder (we load the pre-trained parameters from BART) followed by a GRU decoder.} 


\subsection{High-level Mental Health Summarization}\label{app.method:summary}
We focus on information considered important in summarizing individuals' mental states according to a wide range of therapeutic approaches \cite{eells2022handbook}. Although users broadly talk about mental health related topics in this dataset, each timeline's coverage over clinical concepts varies by nature of differences in individual experience and communication preferences. As such, when annotators write gold summaries and when we generate model-written ones, we focus on  clinical information that is present, ignoring true negatives.

We prompt an instruction-tuned LLM following a multi-stage framework (Fig.~\ref{app.fig:high_level_prompt}) to generate high-level mental health summaries based on timeline summaries. In the \textit{map} stage, we instruct the model to provide inferences based on the timeline summary focusing on clinical topics (Appendix \ref{sec:appendix}, Table \ref{tab:appendix.clinical_concepts}), such as presenting issues, inter/intra-personal patterns, and moments of change (MoC). Instructions and prompts are in Appendix B. In the \textit{reduce} stage, we iteratively prompt the model to combine extracted observations together into a concise summary. 


==> the_version_of_changes/7.results.tex <==
\section{Results}
\label{sec:results}

\subsection{Automatic evaluation}
Table \ref{tab:results.examples} shows example summaries. %For reference-based metrics, we report results averaged over the gold summaries. 
We perform two-tailed permutation tests in our comparisons reporting statistical significance at $\alpha=.05$. 
\begin{table}[]

\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}llrrrr@{}}
\toprule
Aspect & Metric & LLaMA & TH-VAE & Skeleton & Naive \\ \midrule
% salient meaning preservation
SMP 
    & $\text{MHIC}_\text{sem}$ & .65 & \textbf{.66} & .57 & --\\
% factual consistency
\multirow[t]{3}{*}{FC} 
    & $\text{FC}_\text{Timeline}$ & \textbf{.63} & \textbf{.63} & .21 & --\\
    & $\text{FC}_\text{Expert}$ & .95 & \textbf{.96} & .95 & .93\\
 % evidence appropriateness
\multirow[t]{2}{*}{EA} 
    & $\text{EA}$ & \textbf{.97} & \textbf{.97} & .95 & --\\
 % coherence
\multirow[t]{2}{*}{Coherence} 
    & IntraNLI & .95 & \underline{\textbf{.96}} & .95 & .93\\
    & BARTScore & \textbf{-2.96} & -3.10 & -3.09 & --\\
 % fluency
\multirow[t]{2}{*}{Fluency} 
 & $\text{PPL}_\text{Timeline}$ ($\downarrow$) & \underline{\textbf{13.80}} & 56.33 & 31.82 & --\\
 & $\text{PPL}_\text{High-level}$  ($\downarrow$)& 9.32 & \textbf{9.30} & 9.45 & 11.38 \\ \hline 
\end{tabular} 
\end{adjustbox}
\caption{Automatic evaluation for salient meaning preservation (SMP), factual consistency (FC), evidence appropriateness (EA), coherence, and fluency. Higher is better, except for PPL. BARTScore uses log likelihood, hence higher (less negative) is better. Best in \textbf{bold}, significant improvement over second-best \underline{underlined}. %Naive prompting baseline directly produces high-level summaries without an intermediate timeline summary, hence the lack of results on timeline-level metrics.
} 
\label{app.tab:results.auto}
\vspace{-1.5em}
\end{table}
%\noindent\textbf{TH-VAE and LLaMA both capture mental health insights from user timelines, but TH-VAE summaries are more logically coherent.}
TH-VAE and LLaMA generated significantly higher quality summaries compared to other baselines. TH-VAE and LLaMA were comparable on most metrics, preserving mental health information ($\text{MHIC}_{sem}$) while similarly consistent with the source ($\text{FC}_\text{Timeline}$) in timeline summaries and factually consistent with human-written references in high-level mental health summaries ($\text{FC}_\text{Expert}$). 

\textcolor{blue}{Two-tailed permutation tests showed that LLaMA timeline summaries were significantly more fluent ($\text{PPL}_\text{Timeline}$), in line with its tendency to normalise text (see examples, Appendix B). These tests also indicate that high-level summaries were comparably coherent in terms of ease of reading and integrating information from timeline summaries (BARTScore). This is expected since all methods used the same prompting framework to generate high-level summaries. However, TH-VAE achieved significantly higher IntraNLI, suggesting its timeline summaries allow for more logically coherent synthesis of detailed clinical information. }

\subsection{Human evaluation}
We selected three systems for human evaluation: LLaMA, TH-VAE, and the naive LLaMA baseline. This allows us to compare top-performing models and understand how removing timeline summarisation and clinical prompting steps may impact summary quality perceived by human judges.
%As shown in Table \ref{tab:results.likert}, 
TH-VAE produced summaries considered the most factually consistent and useful in summarising changes (MoC) among compared models. Human judges found LLaMA summaries generated with clinical prompts to be most useful in other usefulness criteria, whereas LLaMA with a simple summarisation prompt was consistently least useful. Notably, LLaMA summaries \emph{without} clinical prompts were rated as more factually consistent than those \emph{with} clinical prompts, suggesting they adhered to the source timeline, but were impacted by lack of guidance (Table \ref{app.tab:results.likert}). \textcolor{blue}{A detailed qualitative evaluation in Appendix A.6 shows that Llama timelines present more hallucinations than TH-VAE.}
\begin{table}[!htbp]
\centering
\begin{adjustbox}{width=.82\columnwidth}
\begin{tabular}{@{}lccc@{}}
\toprule 
Aspect                                      & LLaMA & TH-VAE & Naive \\ \midrule
Factual Consistency                         & 3.08 & \textbf{3.35}  & 3.28    \\
Usefulness (General)      & \textbf{3.38} & 3.28  & 2.55 \\
\phantom{---} (Diagnosis) & \textbf{3.40} & 3.25 & 2.93  \\
\phantom{----}(Inter-\& Intrapersonal) & \textbf{3.48}  &  3.33 & 2.23    \\
\phantom{----}(MoC)       & 3.30   &  \textbf{3.35} & 1.18  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Human evaluation results based on 5-point Likert scales (1 is worst, 5 is best). Best in \textbf{bold}.}
\label{app.tab:results.likert}
\vspace{-1em}
\end{table}

\vspace{-0.1cm}
\subsection{Ablation}

\textcolor{blue}{
We performed ablation studies to investigate the importance of key phrases (\S\ref{method:key}) and elaborate clinical prompts for the final summary generation (\S\ref{method:summary}) in TH-VAE and LLaMA. Details are in Appendix \ref{ap:ablation}, Tables~\ref{tab:ablation} and \ref{tab:ablation_llama}.  We experimented with (a) removing keyphrases but keeping the clinical prompts %(`\textit{-keyphrases}') 
and (b) keeping the keyphrases, but prompting the LLM to summarise the high-level summary directly without any guiding topics.} %(`\textit{-clinical prompts}'). 

\textcolor{blue}{In both systems, removing keyphrases results in timeline summaries capturing less salient information ($\text{MHIC}_{sem}$), and degraded logical connectedness ($\text{IntraNLI}$), evidence appropriateness ($\text{EA}$), and factual consistency with gold summaries ($\text{FC}_\text{Expert}$), showing that \emph{keyphrases help focus generation on mental health related information}. In TH-VAE, removing keyphrases made timeline summaries less consistent with the source ($\text{FC}_\text{Timeline}$), and we observed the same trend to a greater effect when clinical prompts are removed. Thus, \emph{the elaborate prompt does provide an efficient clinical guidance for the LLM to generate summaries}.}

\textcolor{blue}{In LLaMA, removing keyphrases improves timeline summary faithfulness ($\text{FC}_\text{Timeline}$) at the expense of clinical information  ($\text{MHIC}_{sem}$). This shows the role of keyphrases guided by domain expertise as anchors in summaries of long texts. Consistency with experts ($\text{FC}_\text{Expert}$) are similar across ablation settings but highest when both are employed, underlining the importance of using these components in conjunction.}
